Quantum Software Ecosystem Design

The rapid advancements in quantum computing necessitate a scientific and rigorous approach to the construction of a corresponding software ecosystem, a topic underexplored and primed for systematic investigation. This chapter takes an important step in this direction: It presents scientific considerations essential for building a quantum software ecosystem that makes quantum computing available for scientific and industrial problem solving. Central to this discourse is the concept of hardware-software co-design, which fosters a bidirectional feedback loop from the application layer at the top of the software stack down to the hardware. This approach begins with compilers and low-level software that are specifically designed to align with the unique specifications and constraints of the quantum processor, proceeds with algorithms developed with a clear understanding of underlying hardware and computational model features, and extends to applications that effectively leverage the capabilities to achieve a quantum advantage. We analyze the ecosystem from two critical perspectives: the conceptual view, focusing on theoretical foundations, and the technical infrastructure, addressing practical implementations around real quantum devices necessary for a functional ecosystem. This approach ensures that the focus is towards promising applications with optimized algorithm-circuit synergy, while ensuring a user-friendly design, an effective data management and an overall orchestration. Our chapter thus offers a guide to the essential concepts and practical strategies necessary for developing a scientifically grounded quantum software ecosystem.

==> figures/workflow.tex <==

\begin{tikzpicture}[thick,xscale=1.1,>=stealth]

    \node[label={[align=center]above:{application\\description}}] (problem) at (0,0) 
        {\usebox{\documentbox}};
    \node[label={[align=center]above:{classical-quantum\\program}}] (classical) at (4,0) 
        {\scalebox{.8}{\usebox{\programbox}}};
    \node[label={[align=center]above:{result}}] (result) at (8,0) 
        {\usebox{\documentbox}};
        
    \node[label={[align=center]below:{quantum\\circuit}}] (circuit) at (4.5,-2) 
        {\usebox{\circuitbox}};
    \node[label={[align=center]below:{circuit\\result}}] (circuit-result) at (7.5,-2) 
        {\scalebox{.75}{\usebox{\documentbox}}};
    
    \path[draw,rounded corners,->] 
        (problem) 
            -- node[fill=white,inner sep=0,label=above:compiler] {\scalebox{.5}{\usebox{\gearbox}}} 
            (classical);
            
    \path[draw,rounded corners,->] 
        (classical) 
            -- node[fill=white,inner sep=0,label={[align=center]above:classical\\system}] (hpc-system) 
                {\scalebox{.5}{\usebox{\serverbox}}} 
            (result);
            
    \path[draw,rounded corners,->] 
        (circuit) 
            -- node[fill=white,inner sep=0,label={[align=center]below:quantum\\computer}] 
                {\scalebox{.75}{\usebox{\quantumbox}}} 
            (circuit-result);
    
    \path[draw,rounded corners,->] 
        ($(hpc-system.south west) + (.25,0)$) 
        |- ($(classical) ! .5 ! (circuit)$) 
        -| ($(circuit.west) - (.5,0)$) 
        -- (circuit);
        
    \path[draw,rounded corners,->] 
        (circuit-result) 
        -- ($(circuit-result.east) + (.5,0)$) 
        |- ($(result) ! .5 ! (circuit-result)$) 
        -| ($(hpc-system.south east) - (.25,0)$);
    
    \path[draw,rounded corners,->] 
        (result) 
        -- ($(result) + (1,0)$) 
        |- (4.5,-3.75) 
        -| node[fill=white,near start] {\usebox{\userbox}} 
            ($(problem) - (1,0)$) -- (problem);

\end{tikzpicture}


==> tex/helpful.tex <==

\bigskip

% \todo[inline]{
%     Please, \\
%     - write a new line for at least each sentence (better for git diff) \\
%     - use \texttt{\textbackslash autoref} for referencing \\
%     - use commands \texttt{\textbackslash eg}, \texttt{\textbackslash ie}, \texttt{\textbackslash etal}
%       and \texttt{\textbackslash cf} for the corresponding abbreviations \\
%     - register abbreviations in \texttt{adds/abbreviations.tex} 
%       and use the corresponding macros in the text \\
%     - add references of your own in \texttt{adds/ours.bib} and of others in \texttt{adds/references.bib} 
%       sorted according to the type (books, articles, preprints, webpages, software) 
%       and in alphabetical order
% }

%\todo[inline]{MF: abbreviations should introduced in the text when they are used the first time - we will not have an abbrevation index in the book itself I think and the book chapter should readable in a closed way anyways}

%\todo{Melven: On overleaf, this is somehow using a bitmap font (pixelated on high resolution)}
    
%\section*{Content}
%\setcounter{minitocdepth}{2}  % remove afterwards
%\dominitoc

%\setglossarysection{section}
%\printabbreviations  % remove afterwards
\clearpage

